Modeling of an ODE-constrained optimization problem describing tumor dynamics, and numerical approximation via sequential physics-informed neural networks

In this paper, we study an optimal control problem related to an ODE model of glioblastoma growth influenced by the oxygen. The model considers a couple of controls describing the chemotherapy and antiangiogenic therapies. The cost functional aims to reduce the tumor growth, bring the oxygen concentration close to a desired value, and penalize the use of therapies. We solve the optimal control problem, proving the existence of a global optimal control and deriving first-order necessary optimality conditions through the Pontryagin Minimum Principle. For the numerical approximation, we use Physics-Informed Neural Networks (PINNs) to solve the state and adjoint systems, together with a gradient descent method with Armijo line search for the controls. To address the strategy of PINNs we consider the methodology proposed in [15], making a decomposition of the time domain into several subintervals, using different neural networks in each subinterval and enforcing continuity conditions between successive time subintervals. This strategy, called sequential PINN formulations in time, including soft and hard-constrained versions, is compared with the corresponding approximation results of classical solvers and traditional PINNs counterparts.

==> graficas/estilos_graficas.tex <==
\ifdefined\GraphStylesCommonLoaded
\else
  \newcommand{\GraphStylesCommonLoaded}{}

  \usetikzlibrary{spy,shadows}
  \definecolor{blueTone}{RGB}{0,76,153}
  \definecolor{redTone}{RGB}{200,0,0}
  \definecolor{greenTone}{RGB}{0,105,65}

  % #1 axis width, #2 axis height, #3 style name A, #4 color A, #5 style name B, #6 color B
  \newcommand{\GraphSetupStyles}[6]{%
    \pgfplotsset{
      axisStyle/.style={
        width=#1,
        height=#2,
        axis line style={draw=black!64, line width=0.28pt},
        tick align=outside,
        tick style={draw=black!62, line width=0.28pt},
        tick label style={font=\footnotesize, text=black!78},
        label style={font=\small},
        xlabel style={yshift=2pt},
        ylabel style={yshift=-1pt},
        title style={font=\small\bfseries, align=center, yshift=1pt},
        grid=both,
        major grid style={draw=black!11, line width=0.24pt},
        minor grid style={draw=black!6, line width=0.18pt},
        minor x tick num=1,
        minor y tick num=1,
        scaled ticks=false,
        y tick label style={
          /pgf/number format/fixed,
          /pgf/number format/precision=3
        },
        enlarge x limits=0.01,
        axis background/.style={fill=white},
        every axis plot/.append style={line join=round, line cap=round, opacity=0.97},
        clip mode=individual
      },
      refStyle/.style={
        color=blueTone,
        line width=0.6pt,
        solid,
        mark=none
      },
      #3/.style={
        color=#4,
        line width=0.8pt,
        dash pattern=on 4.8pt off 2.0pt,
        mark=none
      },
      #5/.style={
        color=#6,
        line width=0.8pt,
        dash pattern=on 1.2pt off 1.7pt,
        mark=none
      },
      legendHidden/.style={
        draw=none,
        fill=none,
        text opacity=0,
        at={(0,0)},
        anchor=south west
      },
      legendBox/.style={
        draw=black!14,
        fill=black!1,
        rounded corners=3pt,
        font=\footnotesize,
        legend cell align=left,
        inner xsep=8pt,
        inner ysep=5pt,
        /tikz/every even column/.append style={column sep=1.2em}
      }
    }
    \tikzset{
      zoomWindow/.style={
        draw=black!70,
        line width=0.8pt,
        fill=white,
        drop shadow={shadow xshift=2.8pt,shadow yshift=-2.8pt,fill=black,opacity=0.35}
      },
      zoomLink/.style={draw=black, line width=0.36pt, opacity=0.38},
      zoomSourceFrame/.style={draw=black, line width=0.45pt, opacity=0.55}
    }
  }
\fi

